Web Services: A Process Algebra Approach

It is now well-admitted that formal methods are helpful for many issues raised in the Web service area. In this paper we present a framework for the design and verification of WSs using process algebras and their tools. We define a two-way mapping between abstract specifications written using these calculi and executable Web services written in BPEL4WS. Several choices are available: design and correct errors in BPEL4WS, using process algebra verification tools, or design and correct in process algebra and automatically obtaining the corresponding BPEL4WS code. The approaches can be combined. Process algebra are not useful only for temporal logic verification: we remark the use of simulation/bisimulation both for verification and for the hierarchical refinement design method. It is worth noting that our approach allows the use of any process algebra depending on the needs of the user at different levels (expressiveness, existence of reasoning tools, user expertise).

==> conclusion.tex <==
\section{Concluding Remarks and future work}
\label{section:cr}

We present a framework, for the design and verification of WSs using process algebras.
We illustrate a two-way mapping between a very expressive process algebra, LOTOS, 
and BPEL. We give also general guidelines for translations between a process algebra and BPEL. 
Process algebra allows not only temporal logic model checking, but also 
a simulation and bisimulation analysis; they allow a design method, hierarchical refinement 
\cite{LS84,Kur94}, that we can apply to WSs. In fact the two-way mapping 
allow us to design and verify both in process algebra and in BPEL.
In Section \ref{section:application}, we sketch how simulation and bisimulation are involved in 
the automatic composition of services and in the redundancy check of services.
In our opinion, these connections deserve to be studied in a future work, together with  
the generalization of the mapping to other languages and 
its implementation. 
In our current mapping, we do not consider dynamic process instantiation and correlation set. 
Moreover we do not tackle the problem of the dynamic choice of the partner to talk to (our interactions
are established before the conversation between partners starts); for this reason we do not consider 
BPEL endpoint references. It is interesting to extend the mapping in these directions.


==> relatedworks.tex <==
\section{Related Works}
\label{section:rw}

We are going to introduce three kinds of related works aiming at: i)
specifying WSs at an abstract level using formal description
techniques and reasoning on them, ii) using jointly abstract
descriptions and executable languages (mainly BPEL), iii) developing
WSs from abstract specifications.

At this abstract level, lots of proposals originally tended to
describe WSs using semi-formal notations, especially workflows
\cite{LeymannVLDB2001}. More recently some more formal proposals
grounded for most of them on transition system models (LTSs, Mealy
automata, Petri nets) have been suggested
\cite{Hull:2003:SLB,Narayanan:2003:ASW,HamadiADC2003,Danielaconficsoc2003,LAPicsoc2003}.
%
With regards to the reasoning issue, works have been dedicated to
verifying WS description to ensure some properties of systems
\cite{Bultan:2004:WWW,Deutsch:2004:PODS,Narayanan:2003:ASW,FosterASE2003,NakajimaOOWS2002}. 
Summarizing these works, they use model checking to verify some
properties of cooperating WSs described using XML-based languages
(DAML-S, WSFL, BPEL, WSCI). Accordingly, they abstract their
representation and ensure some properties using ad-hoc or well-known
tools ({\it e.g.} SPIN, LTSA). We have a deeper look in the following
of this section at proposals focusing on BPEL. 

In comparison to these existing works, the strength of our alternative
approach (using PA) is to work out all these issues (description,
composition, reasoning) at an abstract level, based on the use of
expressive (especially compared to the former proposals) description
techniques and adequate tools. The compositionality property of
process algebra is also very convenient in one area where composition
is one of the main concern. 

The second bunch of related work
\cite{Bultan:2004:WWW,PistoreWSFM2004,FosterASE2003,Narayanan:2003:ASW,ViroliWSFM2004}
deals with mappings between abstract and concrete descriptions of
WSs. Let us emphasize that in first attempts
\cite{prout2004,reportlotos4ws}, we have already proposed some
guidelines to map process algebra and BPEL. Nevertheless, these
guidelines (for CCS and LOTOS)
%focused on precise languages (CCS, LOTOS), they 
were not
defined in details and they deal with a subset of BPEL; in this work 
we include in the mapping also fault, compensation, and event handlers. 
Two relevant related works are
\cite{FosterASE2003,Bultan:2004:WWW}. In the first one, the authors
proposed a formal approach to model and verify the composition of WSs
workflows using the FSP (Finite State Processes) notation and the LTSA
tool. Their paper introduces a translation of the main BPEL structured
activities (sequence, switch, while, pick and flow) into FSP
processes. In the second one, it is presented an approach to
analyze BPEL composite web services communicating through asynchronous
messages. They use guarded automata as an intermediate language from
which different target languages (and tools) can potentially be
employed. They especially illustrate with the use of Promela/SPIN as
the formal language and the corresponding model checker. 
Compared to them, our attempt is more general: 
(i) we show a two-way mapping, useful to develop WSs and also
to reason on deployed ones (the latter direction was the single goal
of mentioned related works). All other previous works 
give only a mapping from BPEL to a formal language. 
(ii) we consider in the mapping also compensation and event handlers, 
and we deal with fault handlers explicitly.
(iii) we can verify not only temporal logic properties, but also 
behaviors equivalences between services using bisimulation. Using this 
facilities we can apply the hierarchical refinement design method to 
WSs, also in the BPEL modelling.

Finally, the recent proposal of Lau
and Mylopoulos \cite{LauICWS2004} argue the use of TROPOS as starting point of 
WS design, but they do not deal with verification, but requirements issues.

% \cite{Bultan:2004:WWW,KimICWS03,PistoreWSFM2004,FosterASE2003,Narayanan:2003:ASW,ViroliWSFM2004} and our previous proposal of course (important to show that in this paper we do more than before) \cite{reportlotos4ws}. And also approaches aiming at developing WSs starting from formal descriptions \cite{LauICWS2004} or not btw, as .NET and J2EE.

